Design of Automatically Adaptable Web Wrappers

Nowadays, the huge amount of information distributed through the Web motivates studying techniques to be adopted in order to extract relevant data in an efficient and reliable way. Both academia and enterprises developed several approaches of Web data extraction, for example using techniques of artificial intelligence or machine learning. Some commonly adopted procedures, namely wrappers, ensure a high degree of precision of information extracted from Web pages, and, at the same time, have to prove robustness in order not to compromise quality and reliability of data themselves. In this paper we focus on some experimental aspects related to the robustness of the data extraction process and the possibility of automatically adapting wrappers. We discuss the implementation of algorithms for finding similarities between two different version of a Web page, in order to handle modifications, avoiding the failure of data extraction tasks and ensuring reliability of information extracted. Our purpose is to evaluate performances, advantages and draw-backs of our novel system of automatic wrapper adaptation.

==> abstract.tex <==
\fontsize{9}{11}\selectfont Nowadays, the huge amount of information distributed through the Web motivates studying techniques to be adopted in order to extract relevant data in an efficient and reliable way. 
Both academia and enterprises developed several approaches of Web data extraction, for example using techniques of artificial intelligence or machine learning.
Some commonly adopted procedures, namely \emph{wrappers}, ensure a high degree of precision of information extracted from Web pages, and, at the same time, have to prove robustness in order not to compromise quality and reliability of data themselves. 

In this paper we focus on some experimental aspects related to the robustness of the data extraction process and the possibility of automatically adapting wrappers. 
We discuss the implementation of algorithms for finding similarities between two different version of a Web page, in order to handle modifications, avoiding the failure of data extraction tasks and ensuring reliability of information extracted. 
Our purpose is to evaluate performances, advantages and draw-backs of our novel system of \emph{automatic wrapper adaptation}. 

==> authors.tex <==
\author{{\textmd {\textbf }}\\
  \fontsize{11}{13}\selectfont
  Emilio Ferrara\\
  \fontsize{9}{11}\selectfont
  \textit{Department of Mathematics, University of Messina, Italy}\\
  \fontsize{9}{11}\selectfont
  \textit{emilio.ferrara@unime.it}\\[12pt]
  %
  \fontsize{11}{13}\selectfont
  Robert Baumgartner\\
  \fontsize{9}{11}\selectfont
  \textit{Lixto Software GmbH, Vienna, Austria}\\
  \fontsize{9}{11}\selectfont
  \textit{robert.baumgartner@lixto.com}\\[12pt]
  %
  % repeat previous group of commands here for further authors
}


==> keywords.tex <==
\fontsize{9}{11}\selectfont Semantic Web, Information Extraction, Data Mining


==> title.tex <==
% The Title is all in Uppercase
\newcommand{\mytitle}{\uppercase{Design Of Automatically Adaptable Web Wrappers} }

